Random Generation and Approximate Counting of Combinatorial Structures

The aim of this thesis is to determine classes of NP relations for which random generation and approximate counting problems admit an efficient solution. Since efficient rank implies efficient random generation, we first investigate some classes of NP relations admitting efficient ranking. On the other hand, there are situations in which efficient random generation is possible even when ranking is computationally infeasible. We introduce the notion of ambiguous description as a tool for random generation and approximate counting in such cases and show, in particular, some applications to the case of formal languages. Finally, we discuss a limit of an heuristic for combinatorial optimization problems based on the random initialization of local search algorithms showing that derandomizing such heuristic can be, in some cases, #P-hard.

==> c0_it.tex <==
\RCSfooter$Id: c0_it.tex,v 1.1 1999/10/29 09:45:54 santini Exp $

\begin{otherlanguage}{italian}
\chapter*{Introduzione}
\label{cha:prefaceit}  

I problemi di conteggio combinatorico hanno una lunga storia; oltre al
loro interesse intrinseco, essi sorgono naturalmente da diverse
investigazioni in numerose branche della matematica e delle scienze
naturali ed hanno dato origine ad una ricca e profonda teoria.  Il
problema del ``ranking'', che consiste nel deteminare la posizione di
un dato elemento di un insieme ben ordinato, è strettamente collegato
al conteggio. I problemi di generazione casuale, viceversa, sono stati
meno studiati ma hanno un grande numero di applicazioni
computazionali.

Dal punto di vista della complessità strutturale, lo studio dei
problemi di conteggio è stato iniziato da \citet{Val79}. Un approccio
parallelo alla generazione casuale è stato propopsto da
\citet*{JVV86}; in particolare, è stato mostrato come la riduzione
usuale dalla generazione al conteggio esatto possa essere modificata
per ottenere un generatore casuale quasi uniforme a partire da stime
approssimate del conteggio. Inoltre, i problemi di generazione casuale
quasi uniforme e conteggio approssimato nel caso generale di \cNP
relazioni\footnote{con \cNP relazioni intendiamo sottoinsiemi
  $R\subseteq\reldom$ tali per cui, comunque presi
  $\alpha,\beta\in\fldom$, si abbia che $|\beta|$ è polinomiale in
  $|\alpha|$ e inoltre il predicato $\alpha\rR\beta$ sia decidibile in
  tempo polinomiale in $|\alpha|$ (dove $\Sigma$ è un fissato alfabeto
  finito).  Per una discussione più accurata, si veda la
  sezione~\ref{sec:prel}.}  sono stati collocati entro il secondo
livello (di una versione probabilistica) della gerarchia polinomiale
~\citep{Sto77}.  In fine, il problema del ``ranking'' è stato studiato
da \citet{Huy90} e da \citet*{GS91} come caso particolare del problema
di compressione ottima.

\bigskip

Obiettivo di questa tesi è stato di determinare classi di \cNP
relazioni per le quali la generazione casuale ed il conteggio
approssimato ammettono una soluzione efficiente. Dal momento che una
soluzione efficiente al problema del ``ranking'' implica che sia
possibile effettuare in modo efficiente anche la generazione casuale,
abbiamo dapprima investigato alcune classi di \cNP relazioni che
ammettessero una soluzione efficiente al ``\emph{ranking}''.  D'altro
canto, ci sono situazioni in cui è possibile ottenere in modo
efficiente la generazione casuale anche quando il problema del
``ranking'' è computazionalmente intrattabile. Abbiamo quindi
introdotto la nozione di ``\emph{descrizione ambigua}'' come strumento
per la generazione casuale uniforme ed il conteggio approssimato in
tali casi e ne abbiamo mostrato, in particolare, alcune applicazioni
al caso dei linguaggi formali. In fine, abbiamo discusso un limite di
una euristica per problemi di \emph{ottimizzazione combinatoria}
basata sull'inizializzazione casuale di algoritmi di ricerca locale
mostrando che la derandomizzazione di tale euristica può costituire un
problema \cnP-difficile. Nei paragrafi che seguono sono descritti in
maggior dettaglio i risultati qui accennati.

\paragraph{Ranking.}

Abbiamo esteso alcuni risultati noti circa il problema del ``ranking''
per i linguaggi formali al caso delle \cNP relazioni. Questo ci ha
consentito di introdurre due nuove classi di relazioni che ammettono
algoritmi di generazione casuale efficienti (\ie che lavorano in tempo
polinomiale). Più precisamente, abbiamo mostrato che le classi di \cNP
relazioni accettate da
\begin{enumerate}[(i)]
\item automi a pila con nastro ausiliario, non ambigui e che lavorano
  in tempo polinomiale;
\item macchine di Turing che lavorano in spazio $s(n)$, con $i(n)$
  inversioni e ambiguità $d(n)$, tali che $s(n)\cdot i(n)\cdot
  d(n)=O(\log n)$,
\end{enumerate}
ammettono una soluzione efficiente al problema del ``ranking''. Tali
risultati seguono dalle tecniche usate rispettivamente da \cite{Huy90}
e \citet*{BMP94} per risolvere l'analogo problema nel caso dei
linguaggi formali. Dal momento che abbiamo inoltre dimostrato che una
soluzione efficiente al problema del ``ranking'' implica l'esistenza
di algoritmi efficienti per la generazione casuale, possiamo
concludere che le \cNP relazioni di suddette classi ammettono
algoritmi di generazione casuale che lavorano in tempo polinomiale.


\paragraph{Ambiguous descriptions.}

To deal with the case in which ranking is computationally infeasible,
we introduce a simple notion of \emph{description} of a combinatorial
structure, together with a corresponding notion of \emph{ambiguity},
and study the problem of uniform random generation and approximate
counting for structures endowed with such descriptions. We prove a
general result stating that if a structure \bS has a description \bT
with polynomially bounded ambiguity and \bT admits a polynomial time
\emph{uniform random generator (\urg)}, then also \bS admits a \urg
working in polynomial time.  If, moreover, the counting problem for
\bT is solvable in polynomial time, then $\bS$ admits a fully
polynomial time \emph{randomized approximation scheme (\ras)} for its
counting problem.  Here, the proofs are based on the Karp-Luby
technique for sampling from a union of sets~\citep{KLM89} and on
Hoeffding's inequality~\citep{Hof63}, a classical tool for bounding
the tail probability of the sum of independent bounded random
variables.  Such general results can be applied to various classes of
languages:
\begin{enumerate}[(i)]
  
\item We show that, for \emph{finitely ambiguous context-free
    languages}, a word of length $n$ can be generated uniformly at
  random in $O(n^2\log n)$ time and $O(n^2)$ space, using $O(n^2\log
  n)$ random bits.  We observe that, in our model of computation, the
  same bounds for time and random bits are obtained for the uniform
  random generation of unambiguous \cf language~\citep{Gol95}.
  Similar bounds are obtained for the corresponding randomized
  approximation scheme. To prove these results we show in detail a
  multiplicity version of Earley's algorithm for context-free
  recognition~\citet{Ear70}. We prove that, for finitely ambiguous \cf
  languages, the number of derivation trees of an input word of size
  $n$ can be computed in $O(n^2\log n)$ time and $O(n^2)$ space;
  
\item We show how to generate, uniformly at random, words from
  languages accepted by \emph{one-way nondeterministic auxiliary
    push-down automata} working in polynomial time and using a
  logarithmic amount of work-space~\citep{Coo70,Coo71,Bra77}.  Also in
  this case, we obtain polynomial time \urg and \ras whenever the
  automaton has a polynomial number of accepting computations for each
  input word.  Observe that such results hold in particular for
  polynomially ambiguous context-free languages.
  
\item We consider the uniform random generation and approximate
  counting of \emph{rational trace languages}~\citep{DR95}.  Finitely
  ambiguous rational trace languages~\citep{BMS82, Sak87} admit \urg
  and \ras of the same time complexity of the algorithms for their
  recognition problem.  Analogously, we obtain polynomial time \urg
  and \ras for the rational trace languages that are polynomially
  ambiguous.

\end{enumerate}



\paragraph{Derandomization and combinatorial optimization.}

We focus our attention on an heuristic suggested by \citet{Gro99} for
improving \emph{local search} algorithms.  The basic idea is to use a
two phase (randomized) algorithm which in a first phase generates
uniformly at random some feasible solution and then, starting from the
best solution so obtained, performs a local search phase. For a large
class of problems, such heuristic is known to give (randomized)
approximation algorithm with a constant performance ratio.  We study
in detail the case in which the objective function of the
combinatorial optimization problem is represented by means of
arithmetic circuits. Sufficient conditions are known in such a case to
prove that the first phase of the heuristic can be ``derandomized''
thus yielding to a deterministic approximation algorithm. By
investigating a problem of transformation between arithmetic circuits,
we bring to light a limit of this approach and show that
``derandomizing'' the first phase of the heuristic, in some cases, is
a \cnP-hard problem.

\end{otherlanguage}



==> c7s1.tex <==
\RCSfooter$Id: c7s1.tex,v 2.1 1999/09/22 17:34:19 santini Exp $

% chapter N
\section{}

% Local Variables: 
% mode: latex
% TeX-master: "master"
% TeX-parse-self: t
% End: 

